Gesture-aware Interactive Machine Teaching with In-situ Object Annotations

Interactive Machine Teaching (IMT) systems allow non-experts to easily create Machine Learning (ML) models. However, existing vision-based IMT systems either ignore annotations on the objects of interest or require users to annotate in a post-hoc manner. Without the annotations on objects, the model may misinterpret the objects using unrelated features. Post-hoc annotations cause additional workload, which diminishes the usability of the overall model building process. In this paper, we develop LookHere, which integrates in-situ object annotations into vision-based IMT. LookHere exploits users' deictic gestures to segment the objects of interest in real time. This segmentation information can be additionally used for training. To achieve the reliable performance of this object segmentation, we utilize our custom dataset called HuTics, including 2040 front-facing images of deictic gestures toward various objects by 170 people. The quantitative results of our user study showed that participants were 16.3 times faster in creating a model with our system compared to a standard IMT system with a post-hoc annotation process while demonstrating comparable accuracies. Additionally, models created by our system showed a significant accuracy improvement ($\Delta mIoU=0.466$) in segmenting the objects of interest compared to those without annotations.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> contents/discussion_old.tex <==
\section{Discussion}
%\koji{}{This section should carefully look back what we have so far including system performance evaluations and dataset as well as results from the user study. What can our work offer to the community as a whole? There must be some things that did not work out or perform well as expected? What are they and why do we think they happened? Discussions on limitations are also necessary.}


\subsection{\revise{Benefits and Limitations of Object Highlights}{}}
\revise{We answer RQ1 through our implementation that demonstrates object highlights guided by users' deictic gestures as illustrated in Figure~\ref{fig:implementation workflow}.
As observed in our results, the object annotations that ware obtained during the teaching process were powerful to reduce participants' workload with achieving accurate models.}{}

\revise{Our evaluation (Section~\ref{sec: techeval}) confirmed that the accuracy of our approach using EfficientNet-b0 and \datasetname was 0.718 ($mIoU$).
While this accuracy was higher than that of the network trained on TEgO-Syn ($mIoU$=0.368), our object highlights}{Despite the effectiveness of our object highlights prove by our user study, they} still had erroneous cases.
% \zhongyi{}{should we put a figure in the main content? or just referring to a figure in the appendix?}
% Figure \xxx shows representative examples where $IoU$ was low (more examples can be found in Appendix~\ref{apdx: failure}). 
For instance, Figure~\ref{fig: pred_failure} shows an example where $IoU$ was low (more examples can be found in Appendix~\ref{apdx: failure}). 
The person in the figure is pointing at an object on her head, but our algorithm incorrectly highlights the clock at the background.
%, which is a visually salient object along the pointing direction in the 2D space.
% \xxx.
% These examples suggest that pointing gestures along the principal axis (the axis from the camera center perpendicular to the image plane) require 3D understanding of a scene for more accurate object region identification.
% Figure~\ref{}
% This is one limitation caused by our current camera configuration.
% A future system could obtain the depth information by using a depth camera, but additional refinements on \datasetname may be necessary.
These failure cases suggest\revise{s}{} a limitation posed by the current implementation using a normal RGB camera because it does not include the depth information of the scene.
%Therefore, our implementation answer to RQ1 contains limitations caused by our design based on the 2D hand segmentation mask, which cannot accurately perceive the object relationship in the 3D world.
A future system may consider obtaining a richer set of information through 3D scene reconstruction~\cite{dahnert2021panoptic}, 3D hand pose estimation~\cite{Cao2021reconstructing, huang2020hand} from RGB images, or use depth cameras~\cite{izadi2011kinect}.
%with additional refinements on \datasetname.
% Recent computer-vision research enables 3D hand pose estimation~\cite{Cao2021reconstructing, huang2020hand} and scene reconstruction~\cite{dahnert2021panoptic}.
% To make
% Importantly, further studies based on these deep architectures should are highly necessary for real-time applications like LookHere.
Future research should further study how to simplify the aforementioned feature extractors to be used in real time for \vimt systems.




% \subsection{Benefits of Integration of Object Annotations into Teaching}
\subsection{In-sit\revise{e}{u} Object Annotations Using Other Approaches}

% \koji{}{We had two RQs. Based on the results we have, how can we answer them?}

% Our evaluations show that our system could support rapid, simple yet accurate human teaching by integrating the fine-graded annotation into the teaching experience.
% My system design principle follows our observation that gestures help
% This work integrates annotations in into human teaching by using implications embedded in human deictic gestures.
% Our implementation is still a first-step solution by following the design principle of the integration.
% The fundamental intuition behind this is that we humans hardly spend many efforts doing annotation tasks in human-human communications, and therefore humans should have a smart way to interactively deliver similar information as we want to collect from annotations.
% Therefore, we envision that future research can innovate more interaction approaches, not limited to our gesture-based one, to achieve the design goal of integration.
% \zhongyi{As we mentioned in Section~\ref{sec: res_qual_advice}, performing different gestural interactions with an object while recording teaching samples may be distracting, causing higher workload.}{revise according to a new result to be added.} 
% Future work can explore diverse methods to integrate annotations into human teaching, and analyze the corresponding benefits to their target applications so that users can easily perform teaching in various use cases.
The results from the user study confirm that LookHere was able to achieve the reduction of workload associated with post-hoc annotations without losing the accuracies of the models created, answering RQ2.
Despite the promising results of LookHere, there are limitations to use deictic gestures while teaching as shown in our qualitative feedback (Section~\ref{sec: res_qual_advice}).
% As suggested by our participants, gestured
% by leveraging users' deictic information in gestures during teaching.
% As our results reveal in Section~\ref{sec: quant_result}, using \systemname does not cause significantly different workload compared to using Na\"{i}veIMT.
% As our results reveal in Section~\ref{sec: result}, participants in our user study highly appreciated the 
% As we show in Section~\ref{sec: result}, our implementation achieves a good integration of annotations with teaching by significantly increasing the segmentation accuracy of the created model and, at the same time, completely removes the post-hoc annotation experiences.
% Nevertheless, we also showed that \systemname causes slight higher workload, despite the unverified significance
% On the other hand, our quantitative and qualitative results show a 
% While our results revealed many benefits of a gesture-aware approach to enable the integration of object annotations into teaching, our solution cannot completely achieve our ultimate goal, i.e., \textit{``users do NOT feel extra workload''}, but that users feel no significant workload difference.
% As is reported in Section~\ref{sec: res_qual_advice}, there were certain limitations in our current answer of the system design, and 
Future work should extend our RQ2 and investigate how other interaction methods or modalities may better support in-situ object annotations.
% While our work validates the benefits of a gesture-aware approach to enable the integration of object annotations into teaching, future work should investigate how other interaction methods or modalities may offer better performance.
As suggested by our participants, a click-based annotation method may be one possibility.
Multi-modal approaches, such as speech input (e.g., mentioning the object of interest by voice), can be another candidate.
This work should serve as a foundation for future research on in-situ object annotation methods in \vimt systems.

% \zhongyi{}{since we've already said that these are future work. I think we can comment out the following two sentences.}
% Such comparative studies are beyond the scope of this work.
% Our work contributes to future studies in user experience of \vimt by introducing a new approach for object annotation that can be executed concurrently with teaching.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/appendix/033-fail-pred.png}
        \caption{Prediction.}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/appendix/033-fail-gt.jpg}
        \caption{Ground truth.}
    \end{subfigure}
    \caption{A failure case of object highlights.}
    \label{fig: pred_failure}
\end{figure}

    

%, implying that there are cases that \systemname cannot accurately presents the highlights. 
% We left in-depth case-based analysis in Appendix~\ref{apdx: failure}.
% In short, our implementation, i.e., using hand segmentation masks, is insufficient to capture the information delivered in humans' gestures.
% For example, pointing gestures can be better perceived in a 3D space rather than a 2D hand segmentation.
% To thoroughly perceive hand-object interactions, we encourage future works to take hand pose detection~\cite{huang2020hand} and 3D scene reconstruction~\cite{dahnert2021panoptic} into considerations during the development.
% We notice one latest work~\cite{Cao2021reconstructing} that studied the problem of hand-object interactions in a 3D space but it currently does not support real-time uses.
% Future work should also simplify the perception model so that it can be used in real time in IMT systems.
% Therefore, 
% Object highlights in \systemname takes an enhanced RGB image by an addition channel of hand segmentation mask as the input to predict the object denoted by human gestures.
% Our object highlights take a hand segmentation mask of an image as gesture-based features to support predictions.
% In reality, hand segmentation masks cannot sufficiently represent the information delivered in humans' gestures.





% We encourage future w

% Future research can also explore more system design ideologies other than our gesture-based ones, providing diverse methods for incorporating annotation into human teaching.

% is still a first-step solution, and encourage future research to outperform our implementation of gesture-aware solutions by using our open-source codes.



% According to our quantitative subject results and various qualitative comments, participants are more satisfied with our efficient design of IMT systems, and believe that similar systems could have a great impact on future society for non-professional uses.
% This verifies our initial hypothesis stated in Section~\ref{sec: hypothesis}.


% Note that we used fundamental ML architectures with the lightest designs (also with the lowest accuracy).
% By utilizing more advanced ML algorithms and fine-grained designs for specific tasks in the future, we could further increase the system performance~\cite{Wu2022Efficient}, bringing an even better user experience.


\subsection{Potential Applications of \datasetname}
One important contribution of this work is the creation of \datasetname.
Although the original objective of this dataset was to enable \systemname, it can be used for a broader range of purposes.
For example, the dataset could be useful to design an intelligent virtual background used in online meeting systems which is aware of the object users are trying to present to others.
Segmentation algorithms for virtual backgrounds do not typically consider the behavior of object holding.
Virtual backgrounds thus often hide the objects held by users, diminishing user experience.
A segmentation method trained using our dataset may resolve this issue effectively.

Similarly, future research may employ our dataset to enable focus effects on objects pointed by users.
Recent smartphones have a capability to generate images with a depth effect (e.g., portrait mode).
With our dataset, a future vision approach may introduce a depth effect to objects users are holding or pointing to.
Like the main purpose of TEgO, our dataset may enable accessible systems for people with visual impairments as well.
We hope that our dataset would encourage researchers and developers to design novel interactive systems.
% For example, it can be applied to virtual background functions in online meetings, since our solution can capture various objects denoted by deictic gestures.
% Existing virtual background technologies only capture ``humans'' and hide all the other objects, and this may affect online communications in which a person wants to share an item held by his/her hand.
% By implementing our solution as a programming patch, such issues can be potentially addressed.
% Additionally, we can foresee the application of our solution into gesture-aware auto-focus functions for photographers.


% \datasetname can also benefit the technology development for the visually impaired. Dataset like TEgO primarily help an algorithm recognize a limited number of daily-life objects held by the user
% (e.g. 19 classes in TEgO).
% Using \datasetname, developers can first locate an object held by the user, and then, on this region of the view, apply a classification model trained on large-scale datasets that cover thousands of object labels (e.g., 1000 classes in ImageNet~\cite{imagenet}).


% \zhongyi{}{HRI Visual impairment. Communication analysis. }
% \subsection{Hel}


% \subsection{something about our hypothesis}
% We envision that future systems embedded with more powerful AI technologies, the system can more accurately capture users' implications under gestures.

% % EfficientVis~\cite{Wu2022Efficient}

% \subsection{Extension to Other Applications}
% \begin{itemize}
%     \item allow the user to clarify the training data in real time without ad-hoc interactions
%     \item ML models can better interpret the teaching concepts even \textit{without} extra human efforts.
%     \item Users can easily learn how to use our system, creating a simple experience for users to upgrade their model through proactive clarification. It also proves that our system design follows human intuitiveness.
    
% \end{itemize}


